Composition Properties of Inferential Privacy for Time-Series Data

With the proliferation of mobile devices and the internet of things, developing principled solutions for privacy in time series applications has become increasingly important. While differential privacy is the gold standard for database privacy, many time series applications require a different kind of guarantee, and a number of recent works have used some form of inferential privacy to address these situations. However, a major barrier to using inferential privacy in practice is its lack of graceful composition -- even if the same or related sensitive data is used in multiple releases that are safe individually, the combined release may have poor privacy properties. In this paper, we study composition properties of a form of inferential privacy called Pufferfish when applied to time-series data. We show that while general Pufferfish mechanisms may not compose gracefully, a specific Pufferfish mechanism, called the Markov Quilt Mechanism, which was recently introduced, has strong composition properties comparable to that of pure differential privacy when applied to time series data.

==> proof_serial_mqm_bn_different.tex <==
\begin{proof}
Consider any secret pair $(X_i=a,X_i=b)$. For $j\in [J]$, let $X_Q^j$ be the best Markov Quilt of $X_i$ used in the $j$-th publishing (with $X_N^j$, $X_R^j$).\\
Let $X_\RQ^j=X_R^j\cup X_Q^j$ for $j\in[J]$. Let $X_N = \cap_{j=1}^{J} X_N^j$, $X_\RQ = \cup_{j=1}^{J} X_\RQ^j$, $X_Q = \cup_{j=1}^{J} X_Q^j$, and $X_R = X_\RQ \backslash X_Q$. 
It is obvious that $X_N$ contains $X_i$, $X_N \cup X_Q \cup X_R = X$ and $X_N, X_Q, X_R$ are disjoint. Since $X_R \subseteq \cup_{j=1}^{J} X_R^j$, we know that \shs{cannot guarantee $X_R$ and $X_i$ is independent given $X_Q$}



, and has size no larger than any $X_N^j$. Also, 



%


$X_\RQ^j=X_R^j\cup X_Q^j$ for $j\in[J]$; let  and $X_\RQ^{} = \cup_{j=1}^{J} X_\RQ^j$. Let , which is guaranteed to contain $X_i$. Note that $X_\RQ^{} \cup X_N^{} = X$. \\
Let $Z_1,\dots, Z_J$ denote the Laplace noises added by \mqm. 
For simplicity, let $x_*$ denote the event that $X_*$ takes value $x_*$.
Then for any $w_1,w_2$, we have
\begin{align}\label{eqn:comp serial main}
&\frac{p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J | X_i=a)}{p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J | X_i=b)} \nonumber\\
=&\frac	{\splitfrac{\int_{x_\RQ^{}} p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J, }
{ x_\RQ^{} | X_i=a) d{x_\RQ^{}}}}
{\splitfrac{\int_{x_\RQ^{}} p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J,}{ x_\RQ^{}| X_i=b) d{x_\RQ^{}}}} \nonumber\\
=&\frac	{\splitfrac{\int_{x_\RQ^{}} p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J|}{ x_\RQ^{}, X_i=a) p(x_\RQ^{}|X_i=a) d{x_\RQ^{}}}}
		{\splitfrac{\int_{x_\RQ^{}} p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J|}{ x_\RQ^{}, X_i=b) p(x_\RQ^{}|X_i=b) d{x_\RQ^{}}}} \nonumber\\
\leq&\max_{x_\RQ^{}}\frac	{\splitfrac{p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J|}{ x_\RQ^{}, X_i=a) p(x_\RQ^{}|X_i=a)}}
{\splitfrac{p(\calF_1(X)+Z_1=w_1,\dots,  \calF_J(X)+Z_J=w_J|}{ x_\RQ^{}, X_i=b) p(x_\RQ^{}|X_i=b)}}.
\end{align}
Firstly consider the first ratio in \eqref{eqn:comp serial main}. Let $X_{N\backslash\{i\}}^{} = X_N^{}\backslash X_{i}$ denote all ``neighbor" nodes except for $X_i$. We have
\begin{align*}
&\frac	{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ^{}, X_i=a)}
		{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ^{}, X_i=b)}\\
=&\frac	{\splitfrac{\int_{x_{N\backslash\{i\}}^{}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2, {x_{N\backslash\{i\}}^{}}|}{ x_\RQ^{}, X_i=a) d {x_{N\backslash\{i\}}^{}}}}
		{\splitfrac{\int_{x_{N\backslash\{i\}}^{}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2, {x_{N\backslash\{i\}}^{}}|}{ x_\RQ^{}, X_i=b) d {x_{N\backslash\{i\}}^{}}}} \\
=&\frac	{\splitfrac{\int_{x_{N\backslash\{i\}}^{}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2|}{{x_{N\backslash\{i\}}^{}}, x_\RQ^{}, X_i=a) p({x_{N\backslash\{i\}}^{}}|x_\RQ^{},X_i=a) d {x_{N\backslash\{i\}}^{}}}}
		{\splitfrac{\int_{x_{N\backslash\{i\}}^{}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2|}{{x_{N\backslash\{i\}}^{}}, x_\RQ^{}, X_i=b) p({x_{N\backslash\{i\}}^{}}|x_\RQ^{},X_i=b) d {x_{N\backslash\{i\}}^{}}}} \\
%
%
=&\frac	{\splitfrac{\int_{x_{N\backslash\{i\}}^{}} p(Z_1=w_1-\calF_1(a,{x_{N\backslash\{i\}}^{}},x_\RQ^{})) p(Z_2=w_2-}{\calF_2(a,{x_{N\backslash\{i\}}^{}},x_\RQ^{})) p({x_{N\backslash\{i\}}^{}}|x_\RQ^{},X_i=a) d {x_{N\backslash\{i\}}^{}}}}
		{\splitfrac{\int_{x_{N\backslash\{i\}}^{}} p(Z_1=w_1-\calF_1(b,{x_{N\backslash\{i\}}^{}},x_\RQ^{})) p(Z_2=w_2-}{\calF_2(b,{x_{N\backslash\{i\}}^{}},x_\RQ^{})) p({x_{N\backslash\{i\}}^{}}|x_\RQ^{},X_i=b) d {x_{N\backslash\{i\}}^{}}}},
\end{align*}
where the last equality follows because $Z_1$ and $Z_2$ are independent given the value of $\calF_1, \calF_2$.\\
Notice that $\calF_1,\calF_2$ can change by at most $\card{X_N^{}} \leq \\ \min\{\card{X_N^{1}}, \card{X_N^{2}}\}$ when $X_\Ni^{}$ and $X_i$ change. So for any ${x_{N\backslash\{i\}}^{}}, {x'_{N\backslash\{i\}}}$,
\begin{align*}
&\frac {p(Z_1=w_1-\calF_1(a,{x_{N\backslash\{i\}}^{}},x_\RQ^{}))} {p(Z_1=w_1-\calF_1(b,{x'_{N\backslash\{i\}}},x_\RQ^{}))} \\
\leq& e^{(\epsilon_1 - e(X_Q^1|X_i))/\card{X_N^1} \times \card{X_N}}\\ \leq& e^{\epsilon_1 - e(X_Q^1|X_i)} \\
&\frac {p(Z_2=w_2-\calF_2(a,{x_{N\backslash\{i\}}^{}},x_\RQ^{}))} {p(Z_2=w_2-\calF_2(b,{x'_{N\backslash\{i\}}},x_\RQ^{}))}\\ 
\leq& e^{(\epsilon_2 - e(X_Q^2|X_i))/\card{X_N^2} \times \card{X_N}}\\ \leq& e^{\epsilon_2 - e(X_Q^2|X_i)}.
\end{align*}
Also, notice that $p({x_{N\backslash\{i\}}^{}}|x_\RQ^{},X_i=a)$, $p({x_{N\backslash\{i\}}^{}}|x_\RQ^{},X_i=b)$ are probability distributions, and ${X_{N\backslash\{i\}}}$ is the random variable we are integrating over on.
Therefore the above ratio is upper bounded by 
\begin{align}\label{eqn:comp serial 1st}
e^{\epsilon_1 + \epsilon_2 - e(X_Q^1|X_i) - e(X_Q^2|X_i)}.
\end{align}
Then we consider the second ratio in \eqref{eqn:comp serial main}.
\begin{align*}
	\frac{p(x_\RQ^{}|X_i=a)}{p(x_\RQ^{}|X_i=b)} 
=&	\frac{p(x_R|x_Q,X_i=a)p(x_Q|X_i=a)}{p(x_R|x_Q,X_i=b)p(x_Q|X_i=b)} \\
=&	\frac{p(x_R|x_Q)p(x_Q|X_i=a)}{p(x_R|x_Q)p(x_Q|X_i=b)} \\
=&	\frac{p(x_Q|X_i=a)}{p(x_Q|X_i=b)} 
\leq	e^{e(X_Q|X_i)},
\end{align*}
where the second equality comes from the fact that $X_Q$ is a Markov Quilt of $X_i$, and the last inequality follows from the definition of \effect.\\
Now we prove that \begin{align}\label{eqn:comp serial together}
e(X_Q^1|X_i) + e(X_Q^2|X_i) =& e(\{X_a,X_b\} | X_i) + e(\{X_a',X_b'\} | X_i) \nonumber\\
\geq& e(\{X_{\max(a,a')}, X_{\min(b,b')}\} | X_i) \nonumber\\
=& e(X_Q | X_i).
\end{align} 
If $X_Q$ is equal to one of $X_Q^1$ and $X_Q^2$, the inequality hold obviously.\\
Otherwise, according to Lemma~\ref{lem:max influence ineq}, we have
\begin{align*}
&e(\{X_a,X_b\} | X_i) + e(\{X_a',X_b'\} | X_i)\\
 \geq& e(X_{\max(a,a')} | X_i) + e(X_{\min(b,b')} | X_i) \\
 \geq& e(\{X_{\max(a,a')}, X_{\min(b,b')}\} | X_i).
\end{align*}
Combining with \ref{eqn:comp serial 1st}, we know that \ref{eqn:comp serial main} is upper bounded by 
\begin{align*}
e^{\epsilon_1 + \epsilon_2 - e(X_Q^1|X_i) - e(X_Q^2|X_i)} e^{e(X_Q|X_i)} \leq e^{\epsilon_1+\epsilon_2}.
\end{align*}
\shs{This may or may not apply to any Baysian network; but I haven't figured it out. I think the \effect\ inequality lemma \ref{lem:max influence ineq} may not hold in this case, because we may not separate \effect\ into parts.}\\
\shs{The same analysis hold for any number of composition. Suppose we have $\{X_Q^j = \{X_{a^j}, X_{b^j}\}\}_{j=1}^k$ as the quilts used in all $k$ runs of \mqm. We can set $X_N$ to be the intersubsection of all $X_N^j$, $X_\RQ$ be the union of all $X_\RQ^j$, and $X_Q = \{X_{\max(\{a^j\})}, X_{\min(\{b^j\})}\}$. Then we still have \eqref{eqn:comp serial together}; basically, apart from the two $X_Q^*$'s each contributing to one side of $X_Q$, other $e(X_Q^* | X_i)$'s are not used. So the bound is still pretty loose; the more runs we have, the looser the bound is.}
\end{proof}

==> proof_serial_mqm_same.tex <==
\begin{proof}
Let $\calF_1$ be $L_1$-Lipschitz and $\calF_2$ be $L_2$-Lipschitz. \\
Consider any secret pair $(X_i=a,X_i=b)$. Let $X_Q$ be the best Markov Quilt of $X_i$ with corresponding $X_R,X_N$. Let $X_\RQ=X_R\cup X_Q$, and $x_\RQ$ be any realization of it. Let $Z_1\sim\Lap(\sigma^1),Z_2\sim\Lap(\sigma^2)$ denote the Laplace noises added by \mqm. 
If \mqm\ use the same Markov quilts $X_Q$ on $X_i$ for both publishes, then we know that $\sigma^1 \geq \frac{L_1 \card{X_N}}{\epsilon - e(X_Q |X_i)}$, $\sigma^2 \geq \frac{L_2 \card{X_N}}{\epsilon - e(X_Q |X_i)}$.\\
For simplicity, let $x_*$ denote the event that $X_*$ takes value $x_*$.
Then for any $w_1,w_2$, we have
\begin{align}\label{eqn:comp serial main}
&\frac{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2 | X_i=a)}{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2 | X_i=b)} \nonumber\\
=&\frac	{\int_{x_\RQ} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2, x_\RQ| X_i=a) d{x_\RQ}}
		{\int_{x_\RQ} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2, x_\RQ| X_i=b) d{x_\RQ}} \nonumber\\
=&\frac	{\int_{x_\RQ} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ, X_i=a) p(x_\RQ|X_i=a) d{x_\RQ}}
		{\int_{x_\RQ} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ, X_i=b) p(x_\RQ|X_i=b) d{x_\RQ}} \nonumber\\
\leq&\max_{x_\RQ}\frac	{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ, X_i=a) p(x_\RQ|X_i=a)}
						{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ, X_i=b) p(x_\RQ|X_i=b)}.
\end{align}
Firstly consider the first ratio in \eqref{eqn:comp serial main}. Let $X_{N\backslash\{i\}}$ denote all ``neighbor" nodes except for $X_i$. We have
\begin{align*}
&\frac	{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ, X_i=a)}
		{p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2| x_\RQ, X_i=b)}\\
=&\frac	{\int_{x_{N\backslash\{i\}}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2, {x_{N\backslash\{i\}}}| x_\RQ, X_i=a) d {x_{N\backslash\{i\}}}}
		{\int_{x_{N\backslash\{i\}}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2, {x_{N\backslash\{i\}}}| x_\RQ, X_i=b) d {x_{N\backslash\{i\}}}} \\
=&\frac	{\int_{x_{N\backslash\{i\}}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2|{x_{N\backslash\{i\}}}, x_\RQ, X_i=a) p({x_{N\backslash\{i\}}}|x_\RQ,X_i=a) d {x_{N\backslash\{i\}}}}
		{\int_{x_{N\backslash\{i\}}} p(\calF_1(X)+Z_1=w_1, \calF_2(X)+Z_2=w_2|{x_{N\backslash\{i\}}}, x_\RQ, X_i=b) p({x_{N\backslash\{i\}}}|x_\RQ,X_i=b) d {x_{N\backslash\{i\}}}} \\
%
%
=&\frac	{\int_{x_{N\backslash\{i\}}} p(Z_1=w_1-\calF_1(a,{x_{N\backslash\{i\}}},x_\RQ)) p(Z_2=w_2-\calF_2(a,{x_{N\backslash\{i\}}},x_\RQ)) p({x_{N\backslash\{i\}}}|x_\RQ,X_i=a) d {x_{N\backslash\{i\}}}}
		{\int_{x_{N\backslash\{i\}}} p(Z_1=w_1-\calF_1(b,{x_{N\backslash\{i\}}},x_\RQ)) p(Z_2=w_2-\calF_2(b,{x_{N\backslash\{i\}}},x_\RQ)) p({x_{N\backslash\{i\}}}|x_\RQ,X_i=b) d {x_{N\backslash\{i\}}}},
\end{align*}
where the last equality follows because $Z_1$ and $Z_2$ are independent given the value of $\calF_1, \calF_2$.\\
Notice that $\calF_1,\calF_2$ can change by at most $L_1\card{N}$ and $L_2\card{N}$ when $X_{N\backslash\{i\}}$ and $X_i$ change. So for any ${x_{N\backslash\{i\}}}, {x'_{N\backslash\{i\}}}$,
\begin{align*}
&\frac {p(Z_1=w_1-\calF_1(a,{x_{N\backslash\{i\}}},x_\RQ))} {p(Z_1=w_1-\calF_1(b,{x'_{N\backslash\{i\}}},x_\RQ))} \leq e^{\epsilon_1 - e(X_Q|X_i)} \\
&\frac {p(Z_2=w_2-\calF_2(a,{x_{N\backslash\{i\}}},x_\RQ))} {p(Z_2=w_2-\calF_2(b,{x'_{N\backslash\{i\}}},x_\RQ))} \leq e^{\epsilon_2 - e(X_Q|X_i)}.
\end{align*}
Also, notice that $p({x_{N\backslash\{i\}}}|x_\RQ,X_i=a)$, $p({x_{N\backslash\{i\}}}|x_\RQ,X_i=b)$ are probability distributions, and ${X_{N\backslash\{i\}}}$ is the random variable we are integrating over on.
Therefore the above ratio is upper bounded by 
\begin{align}\label{eqn:comp serial 1st}
e^{\epsilon_1 - e(X_Q|X_i)} e^{\epsilon_2 - e(X_Q|X_i)}.
\end{align}
Then we consider the second ratio in \eqref{eqn:comp serial main}.
\begin{align*}
	\frac{p(x_\RQ|X_i=a)}{p(x_\RQ|X_i=b)} 
=&	\frac{p(x_R|x_Q,X_i=a)p(x_Q|X_i=a)}{p(x_R|x_Q,X_i=b)p(x_Q|X_i=b)} 
=	\frac{p(x_R|x_Q)p(x_Q|X_i=a)}{p(x_R|x_Q)p(x_Q|X_i=b)} \\
=&	\frac{p(x_Q|X_i=a)}{p(x_Q|X_i=b)} 
\leq	e^{e(X_Q|X_i)},
\end{align*}
where the second equality comes from the fact that $X_Q$ is a Markov Quilt of $X_i$, and the last inequality follows from the definition of \effect.\\
Combining with \ref{eqn:comp serial 1st}, we know that \ref{eqn:comp serial main} is upper bounded by 
\begin{align*}
e^{\epsilon_1 - e(X_Q|X_i)} e^{\epsilon_2 - e(X_Q|X_i)} e^{e(X_Q|X_i)} \leq e^{\epsilon_1+\epsilon_2}.
\end{align*}
\end{proof}
